Discovering Flaws in Security-Focused Static Analysis Tools for Android using Systematic Mutation

Mobile application security has been one of the major areas of security research in the last decade. Numerous application analysis tools have been proposed in response to malicious, curious, or vulnerable apps. However, existing tools, and specifically, static analysis tools, trade soundness of the analysis for precision and performance, and are hence soundy. Unfortunately, the specific unsound choices or flaws in the design of these tools are often not known or well-documented, leading to a misplaced confidence among researchers, developers, and users. This paper proposes the Mutation-based soundness evaluation ($\mu$SE) framework, which systematically evaluates Android static analysis tools to discover, document, and fix, flaws, by leveraging the well-founded practice of mutation analysis. We implement $\mu$SE as a semi-automated framework, and apply it to a set of prominent Android static analysis tools that detect private data leaks in apps. As the result of an in-depth analysis of one of the major tools, we discover 13 undocumented flaws. More importantly, we discover that all 13 flaws propagate to tools that inherit the flawed tool. We successfully fix one of the flaws in cooperation with the tool developers. Our results motivate the urgent need for systematic discovery and documentation of unsound choices in soundy tools, and demonstrate the opportunities in leveraging mutation testing in achieving this goal.

==> approach-design.tex <==
\section{Approach Design}
\label{sec:appraoch}

\begin{figure}[t]
	\vspace{-2em}
    \centering
    \includegraphics[width=\linewidth]{figs/expanding_core} 
    \vspace{-1em}
    \caption{{\small Through systematic evaluation, \tool will discover
    unsound assumptions in security tools, and assist developers and
    researchers in expanding the sound core of their technique towards
    sound analysis.}} 
\vspace{-1em}
\label{fig:expanding_core}
\end{figure} 
In this section we outline our Mutation-based Security Evaluation (\tool) of Android
security tools that use static analysis.  As shown in Figure~\ref{fig:expanding_core}, \tool
starts with a given security tool that has a sound core, but which makes
some unsound assumptions, resulting in a sound{\em y} analysis. \tool
evaluates the tool by executing it over mutants, \ie apps to
which security mutation operators (\ie\ {\em security operators})
designed for a given tool are applied per the {\em mutation
scheme}, which governs the implementation and placement of the
operators in the app (\ie making them mutants). %\DENYS{This is a bit loaded
%sentence, we possibly need to refactor it}
%\ADWAIT{I changed ``in the context of the security'' to ``in the
%application''. Does this make it less complex?}
The security
operators represent anomalies that the static analysis tools are
expected to detect. The undetected mutants indicate likely deficiencies
in the tool, which leads to the broader discovery and awareness of the
unsound assumptions of the tools in the least, and should eventually
facilitate the stakeholders to fix the technique and
expand the sound core. Our approach is organized into two major phases: (i) derivation of security operators, and (ii) implementation of the mutation scheme. 


% Phase 1: Basic ``image'' of the proposal
% Task: Implementing mutations
\begin{comment}
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figs/tasks}
  \vspace{-1.5em}
  \caption{{\small Proposed roadmap of research tasks.}} 
  \label{fig:roadmap}
\end{figure}
\end{comment}

\begin{comment}
The first phase of \tool concerns
the derivation of security operators. Our initial focus will be on
building a comprehensive taxonomy of Android static analysis tools,
characterized by the security goal (\eg detecting data leaks, SSL
vulnerabilities) behind them ({\em Task 1}). In addition to providing
insight into the diverse array of security goals that are supported by
static analysis tools, this taxonomy will also describe the dependencies
between tools, and hence, the potential propagation of vulnerabilities.
For each branch of this taxonomy, we will then derive specifications for
mutation operators for security (\ie the security operators), using a
combination of manual and automated analysis of research artifacts such
as papers, tool manuals and documentation, security bug reports and
issues in app repositories, and other relevant resources ({\em
Task 2}).  However, the derived security operator specifications can be
instantiated differently based on the tool (or type of the tool) being
evaluated. Thus, we will develop a mapping of the operator
specifications to one or more relevant tool types from the taxonomy to
which they apply ({\em Task 3}), to provide an input to the
instantiation in the next phase of the research.
%and then define a methodology for
%instantiating security operators from their specifications, in the
%context of the security tool being evaluated ({\em Task 4}).

% Step 2
The second phase of our research (RG$_2$) explores strategies to improve
the practical applicability of \tool. First, we will investigate methods
to precisely instantiate the security operators in the context of the
security tool under evaluation, by using the context derived from the
tool itself ({\em Task 4}). Further, a simple baseline mutation scheme
would support trivial placement of mutations in apps, \ie it
would consider the security operator instances generated from
{\em Task 4}, and place them at easily reachable locations (\eg the
beginning of the main method). Such
trivial placement is often discouraged in mutation testing for
functional bugs, and may not be sufficient for a reliable
security evaluation. Since this proposal targets the soundness of
security techniques, we will create mutation placement strategies that
consider the adversary model (\eg vulnerability in a benign/curious
app, or malware) as the primary factor in deciding mutation placement
({\em Task 5}). Note that the mutation scheme, \ie operator
instantiation as well as placement, is always specific to the context of
the type of tool being evaluated (\eg data leak detection,
inter-app data flow detection).  %\ADWAIT{@Denys: Any better way
%to say the next sentence?} 
%Therefore, in the interest of a tractable research agenda, our research will use data leak detection tools (\eg FlowDroid~\cite{arf+14}) as a case study, and investigate mutation schemes within the scope of this particular popular class of techniques.
In this proposal we will focus on analyzing data leak detection
tools (\eg FlowDroid~\cite{arf+14}), and investigate
mutation schemes within the scope of this popular class of
techniques.  

In parallel, we will use existing metrics to evaluate the
effectiveness of the mutation schema, and extend existing metrics or
invent new ones if required, since our use of security operators is in a
different context than the general use of functional mutation operators
({\em Task 6}).  This final task will not only assist in achieving our
research objectives, but also make broad contributions to the field of
mutation testing.


% Step 3
The third phase of our research (RG$_3$) will explore the utility as
well as the limitations of \tool. We will first use \tool to evaluate the
soundness of widely-used static analysis tools that detect data leaks in
Android apps ({\em Task 6}). Moreover, we will report the
undetected mutants to the tool developers, and assist them in the resolution
of the actual unsound assumption(s) behind found vulnerabilities, and the
development of patches ({\em Task 7}). Finally, we will leverage the
experience in using \tool for improving real security techniques for
refining our security operators and mutation policies, and explore the
generality of \tool by adapting our methodology to another type of
security tool; \eg those that detect SSL vulnerabilities ({\em Task
8}). 
\end{comment}


\subsection{Derivation of Security Operators}
\label{sec:operators}

Deriving a rich set of security-related mutation operators ({\em  security operators}) is a key component of \tool. We propose a systematic, data-driven methodology to design the security operators (\ie to derive their specifications) following which they will be implemented in the context of individual tools (Section~\ref{sec:mutation_scheme}). Our plan to accomplish this consists of the following three tasks: (i) generating a taxonomy of security research tools focused on static analysis of Android apps, (ii) deriving security operator specifications using the taxonomy, and (iii) mapping security operators back to tools in the taxonomy, to facilitate context-specific instantiation within \tool. 

When designing security operators for evaluating security tools, an
important question is, {\em what should these operators express?}  Just
as mutants in software testing are abnormalities that the test suite
must detect, we envision that security operators must express unwanted
app functionality representing vulnerabilities or malware, that security
tools should detect. Thus, a good starting point is specifying security
operators based on the claims made by various security tools themselves;
\ie security tools must definitely detect the app functionality that
they claim to detect, unless affected by some unsound design choice that
hinders detection. These claims, consisting of descriptions of abstract
programmatic patterns in end-user apps, will form our first type of
security operator specifications.  
\begin{comment}
In addition to claims made by security techniques, bug reports in the
security tools themselves as well as open source apps are another
potential source of security operators, as existing security bugs may
already be under the purview of some Android security static analysis
technique. As a result, security bugs in apps can be a potentially
valuable source of specifications for security operators, just as
functional bugs reported in open source apps can be used to model
mutation operators for more traditional software testing. In summary, we
plan to systematically extract a comprehensive set of security operators
for evaluating Android static analysis techniques using \tool, using
(i) claims made by existing tools (\ie from a detailed taxonomy)
and their known security issues/assumptions, and (ii) security bugs
in open source apps.
\end{comment}


%--------------Task-1----------------
\subsubsection{Tool Taxonomy}
To apply \tool to security-focused static application analysis tools, we
first need to derive a taxonomy of existing security analysis tools for
Android that rely on static analysis. We have
developed an initial taxonomy of security-focused static program
analysis tools using the expert knowledge of the PIs and an initial
literature review. For some techniques we have also begun augmenting
this broad taxonomy with the prevalence of these tools, their lineage
(\ie if they extend another tool), as well as some of their functions
and known assumptions. %For instance, in our preliminary work in
%Section~\ref{sec:preliminary}, we used a rudimentary taxonomy to
%discover that the vulnerability in FlowDroid was generally not discussed
%in all of the 13 research tools extending it.  
\begin{comment}
This initial taxonomy illustrates the prevalence of
these tools, their lineage (\ie if they extend another tool in the
taxonomy), as well as some of their functions, known assumptions, and
limitations. This initial taxonomy is described in detail in
Section~\ref{sec:preliminary}.\TODO{@Richie, anything else to add here?}
%\DENYS{I guess we can just put a few sentences here from Richie's
analysis of the related work}
\end{comment}


%\DENYS{We need to summarize this in one average size paragraph}
%We plan to significantly expand our initial taxonomy in terms of both breadth
%(\ie tool types) and depth (\ie lineage and other information)
%We define a rigorous literature review methodology that can function iteratively over time, with new tools being added and classified according to the taxonomy.  Additionally, we will publish this taxonomy in a public GitHub repository, allowing other researchers or security analysts to contribute. %\ADWAIT{Is ``instantiate this taxonomy in a version control system'' necessary? Too much detail?}
%The attributes upon which the identified tools are classified will allow for the identification of claims of functionality that will later be tested by \tool via the specification, instantiation and execution of security operators. The literature review will be carried out in accordance with the guidelines by Kitchenham \etal, which breaks down the  review process into the steps of (i) identification of the need for the review; (ii) definition of research questions,  (iii) search strategy, (iv) study selection process, (v) data extraction, and (vi) data synthesis \cite{Kitchenham:07}. The end result will be a \textit{tool taxonomy} that stipulates (among other attributes) the high-level functional claims, in terms of information detected via the static analysis, made by each tool. This is the first type of security operator specification that we will define. %We describe our proposed procedure for each of these steps below. %\DENYS{I think we need to mention *Droid survey somewhere in this context?} \ADWAIT{The *Droid paper was not really as thorough as Sufatrio, so we can ignore it.} \TODO{@Kevin: I really like these steps; however, they take up a lot of room. Can we describe each point in one single sentence, and not enumerated, but in a paragraph? We could save some space here.}

	%While similar literature reviews on this topic exist \cite{Sufatrio:ACM15}, none explicitly aim to extract and derive a taxonomy in the detail required  to derive security operator specifications.  Thus the main need is to describe in detail the claims and assumptions of the studied tools. We will investigate three primary research questions (RQs) during the course of this literature review -- \textbf{RQ$_1$}: What are the current goals of  static analysis tools for Android applications? \textbf{RQ$_2$}: What are the claimed functionalities of each of these tools? \textbf{RQ$_3$} What are the assumptions, shortcomings, and fundamental limitations associated with these tools? To ensure the inclusion of as many relevant papers as possible in our literature we will carefully craft a search strategy using an iterative methodology.  We will limit our search to online databases of peer reviewed journals and conference proceedings from top academic conferences in computer security and software engineering. Such venues include, but are not   limited to, IEEE S\&P, ACM CCS, the USENIX Security Symposium, NDSS, ACSAC, WiSec, ICSE, FSE, ASE, ISSTA, TSE, EMSE, We will develop multi-faceted search strings using boolean logic to fine-tune results from relevant digital libraries. We will limit our focus to approaches for static program analysis of Android applications published since 2007 (\ie Android was introduced in 2007). Only studies describing static program analysis for Android will be considered. For each paper describing an Android-focused static analysis tool resulting from our study we will extract information corresponding to the RQs designated above.  After the data extraction process the   PIs and their students as well as their collaborators (see support   letters) will synthesize the data into discrete summaries along each RQ, forming a taxonomy of tools that will help guide the process of deriving security operator specifications.


 %--------------Task-2----------------
\subsubsection{Deriving Operator Specifications}

%\ADWAIT{@Kevin: Revise this paragraph. Only include the motivation, minus the details of proposed work that we will describe later. Also, a lot of this motivation is at the beginning of 4.1; simply abstracting it into 1-2 sentences should be okay.}

%\ADWAIT{@Kevin: The motivation behind looking at adversarial implementations is that it will help the instantiation. However, piggybacking it with this task is more efficient. So, you can say that exactly this, and the reviewer will not mind that it looks so different from the rest of the proposed work, and you won't have to justify it so much later.}

%\ADWAIT{@Kevin: As described before, separate this malware part, make it a brief introduction, and bring it up after completely describing the top-down and bottom up portions.}

	%To derive our taxonomy of operator specifications we will
	%manually extract and analyze information from two
	%\textit{complimentary} sources of information, (i) reported
	%capabilities and assumptions of tools, and (ii) security issues
	%reported in the issue tracker of open source Android apps
	%hosted on GitHub.  Reported capabilities for existing tools
	%will allow for the creation of operators that can test claimed
	%functionalities, as discussed at the beginning of Sec. 4.   
	%\ADWAIT{@Kevin: Make sure the first sentence, i.e., the two {\em
	%complimentary} sources are consistent with what we describe at
	%the beginning of Section 4.1 as stated}
%As stated at the beginning of Sec 4.1, we will utilize two
%{\em complimentary} sources of information in our empirical study to
%derive operator specifications: (i) reported capabilities and claims of
%security tools and the security issues reported in them, and (ii)
%security issues reported in the issue trackers of open source Android
%apps hosted on GitHub.

\begin{comment}
First, the corpus of tool functionality claims
should serve as an effective information source to model security
operators testing purported program analysis functionalities.  However
we must also consider \textit{naturally occurring} security bugs that
arise in open source apps, as such bugs may fall under the range of
detection capabilities of the studied tools.
\end{comment}
%Thus, we will also examine the issue trackers of open source Android
%app hosted on GitHub with the intent of categorizing reported security
%bugs, similar to the co-PI's past work \cite{lbt+17}.  
%These two complimentary information sources should lead to the creation
%of a broad set of definitions or specifications to guide the
%instantiation of security operators.  

%We will accomplish this by both (i) leveraging properties and configurations of the studied tools (Sec. 4.2), and via (ii) utilizing adversarial implementation examples of our derived operators existing in known Android malware.  Additionally, studied malware examples have the potential to define new operator specifications not observed in the first two sources of information.  We label the examination of this final data source of malicious apps, an \textit{augmentation} approach as it builds upon our initial two sources of security operators.

	%As outlined at the beginning of Sec. 4, our derivation of security operator specifications will stem from two primary information sources: (i) claims of tool functionality (\ie Top-Down), and (ii) existing security bugs in open source Android applications (\ie Bottom-Up).  As a result of our systematic literature review from {\it Task 1}, we will already gain a large taxonomy of claimed tool functionalities, however, these tools may have evolved over time to add new features and analyses, or certain features may have been absent from their description in the related publication.  Additionally, surveying known limitations or assumptions that these tools make may lead to previously unreported assumptions that cross-cut other tools.  Thus, we plan to mine the open source issue trackers of these static analysis tools in order to extract further functional claims and reported limitations or assumptions.  In addition to tool functionalities, we also aim to leverage existing security bugs occurring ``in-the-wild" reported to the issue trackers of open source applications that could be effectively abstracted to security operators.  After empirically analyzing these two information sources, we will gain a set of high-level labels describing both tool functionality and real security bugs representing {\it security operator specifications}.  However, there are many different manners in which these specifications can be instantiated. For instance, a functional claim of a tool may be ``capable of detecting information sent over the network", but there are countless variants in which such a concept could be expressed as a mutation operator.  One option, which we describe in detail in Sec. 4.2, is using various properties of the studied tools to configure the operator instantiation. However, in order to form strong operators, it is best to assume an adversarial stance to the studied tools, to more rigorously evaluate their capabilities. Thus, in addition to information directly related to tools, we also propose to examine existing instances of apps that exhibit malicious behavior and/or vulnerabilities. Affected code regions exhibiting risky or malicious behavior can then be linked to the functionalities and security bugs already established and treated as adversarial examples of these concepts which can be used to aid the mutant instantiation process described in Sec. 4.2.
\begin{comment}
Co-PI Poshyvanyk has extensive recent
experience in empirically deriving mutation operators for Android
apps.  In a recent paper, his group introduced
\mdroid~\cite{lbt+17}, a mutation framework specifically tailored for
the functional testing of Android apps~\cite{lbt+17}.  \mdroid was empirically derived through a large-scale study where
eight researchers examined six different sources of information (\ie
which were semi-automatically mined and coded using software
infrastructure developed by the co-PI) in order to derive a detailed
taxonomy of Android bugs that naturally occur in the wild.  This
taxonomy was then used to derive 38 new mutation operators designed to
more effectively measure the efficacy of Android test-suites against
commonly observed bugs.  
%The empirical study examined six different sources of information (\eg
%closed issue reports, bug fixing commits) which were automatically or
%semi-automatically mined using software infrastructure developed by the
%PIs, and was then formatted and imported into a custom-built web-app
%that facilitated the open-coding of the mined information
%This allowed for the subsequent construction of the Android
%fault-taxonomy. 
Similar techniques as well as the infrastructure developed in this prior
work by the co-PI work will be revised and leveraged to fulfill this task.
\begin{comment}
\myparagraph{Preliminary Work} Co-PI Poshyvanyk has extensive recent
experience in empirically deriving mutation operators for functional
testing of Android Applications.  In a recent paper, his group
introduced \mdroid \cite{lbt+17}, a mutation framework specifically
tailored for the functional testing of Android applications
\cite{lbt+17}.  This framework was empirically derived through a
large-scale empirical study where eight researchers examined six
different sources of information in order to derive a detailed taxonomy
of Android bugs that naturally occur in the wild.  This taxonomy was
then used to derive 38 new mutation operators designed to more
effectively measure the efficacy of Android test-suites against commonly
observed bugs.  The empirical study examined six different sources of
information (\eg closed issue reports, bug fixing commits) which were
automatically or semi-automatically mined using software infrastructure
developed by the PIs.  This information was then formatted and imported
into a custom-built web-app that facilitated the open-coding of the
mined information, allowing for the subsequent construction of the
Android fault-taxonomy. 
\end{comment}

%Our work on deriving a taxonomy of \textit{security operators} for Android static analysis tools will leverage the PI's experience in rigorously conducting a large-scale empirical study involving unstructured data, including the software infrastructure for mining software repositories (MSR) and the custom-designed web app to facilitate effective, efficient open-coding. 
%These 38 operators were instantiated in a tool called \mdroid that functions by first extracting a \textit{potential fault profile (PFP)} from a target application to be analyzed. It then seeds mutants into the app in all possible locations as stipulated in the PFP.    \ADWAIT{@Kevin: I think we have motivated it enough. Directly jump into the proposed work now.}

%\ADWAIT{@Kevin: Also, I think the budget for this proposed work should be 0.75 of the page, MAX. Describe them both.}

%\ADWAIT{@Kevin: After top-down and bottom-up have been described, then quickly introduce and describe the analysis of malware samples to aid instantiation.  Separating it helps with the context switch.}

%\ADWAIT{@Kevin: Recall sources in 1 sentence. Then, introduce ``top-down'' and ``bottom-up'' in one/two sentences each. }
\begin{comment}
To derive operator specifications, we conducted an empirical study in a
semi-automated fashion, where information was automatically
extracted from each source, formatted into discrete chunks we refer to
as ``documents", and then manually analyzed and tagged by the authors and
students.  The collected data will be manually
analyzed following a procedure inspired by open coding~\cite{Miles2013},
supported by a custom-built web-app, as in the prior work \cite{lbt+17}. 
Because we start with reported functional claims and
limitations directly coupled to specific tools, we refer
to the process of coding this information, both in the literature review
and empirical study, as a  {\em top-down} process.  For the security
bugs in open source projects, because this process starts with
apps that have no direct coupling to the program analysis tools we are
studying, we label this analysis as {\em bottom-up}.  %Finally,
%we identify adversarial implementations of security operators to {\em
%augment} the specifications generated, aiding instantiation. 
We will we extract documents from the following sources:
%\DENYS{I think we need to have one sentence for each source here and
%list sources in italic inlined in text rather than bold?}
%\KEVIN{@Denys, not sure what you mean by this comment?}
%\ADWAIT{@Kevin: These details are okay here. Therefore, in the first proposed work paragraph, remove these details and only introduce top-down and bottom-up in 1-2 sentences each}
\end{comment}

%\noindent {\bf Reported Tool Capabilities and Limitations ({\em
%Top-Down})}: 
%Issue reports are the most obvious source to mine in order
%to identify additional claims of functionalities and security problems
%that underline Android security tools.  
To derive our set of security operators, we have created a corpus of tool functionality claims, in
order to specify security operators testing purported program analysis
functionalities.  We also examined the issue trackers of Android
security tools identified in our {\em tool taxonomy} from their
respective repositories. We sampled {\em both} closed and
open issues, as we were interested in extracting as many potential issues
as possible to derive the operator specifications. The issue description
thread will then be utilized for the open coding process;
%\end{enumerate}
\begin{comment}
\noindent \textbf{Existing Security Bugs (\textit{Bottom-Up}):} 
We will also mine the issue trackers of open source Android apps
hosted on GitHub. Such apps will be identified by locally cloning all
Java projects ($\approx$ 380,000 of which have already been mined by the
PIs) indicated through GitHub's API. 
% and then filtering for projects containing an \texttt{\small
% AndroidManifest.xml} file (a requirement for Android apps). 
 We will then remove forked projects to avoid duplicated apps and filter
 projects that did not have a single star or a watcher to avoid
 abandoned (or toy) projects. 
 %Once the repository URLs have been identified we will utilize a web
 %crawler to mine the GitHub issue trackers.  Since we are interested in
 %as many potential security bugs as possible, we will consider both
 %closed and open issues containing the ``Bug" or ``Security" tags. 
 We will use a web crawler to mine the GitHub issue trackers for as many
 potential security bugs as possible, thus considering both closed and
 open issues containing security-related tags.  The issues threads will
 be formatted as documents for the online tagging application. We will
 not limit our analysis to the issue description, but will also analyze
 (i) the entire discussion by the developers, (ii) the commit
 messages related to the bug fixes, and (iii) the patches used to fix the
 bugs (\ie source code diff). 
 %To do this, we will utilize the \emph{git} command line utility to extract the commit notes and matched the ones containing lexical patterns indicating bug fixing activities, \eg {\em ``fix issue''}, {\em ``fixed bug''}, similarly to the approach proposed by Fischer \etal \cite{FischerPG03}.
%\end{enumerate}
\end{comment}

In addition to deriving operator specifications from tool claims and issues, we also leveraged an opportunity to extract potential adversarial examples of
operators in a data-driven manner. That is, there may be various ways in
which the operators can be instantiated (\ie in terms of the code
semantics), and our adversarial stance is aimed at creating robust
operator instantiations which are more likely to find hidden assumptions
contributing to the sound\emph{i}ness of the analysis tools. %The PIs have
currently obtained access to two widely-used sources of Android Malware:
%the Android Malware Genome Project~\cite{zj12} (1,260 samples) and the
%Android Malware Dataset~\cite{wlr+17} (24,553 samples), which will be
%used to extract malware descriptions, application code, and other
%metadata into the open coding web-app. This set of adversarial operator
%instantiations will add expressibility to the task of instantiating
%context-specific operators in {\em Task 4}.

\begin{comment}
While the specifications derived from these sources are likely to serve
as a strong base for implementing security operators, there may be
various ways in which the operators can be instantiated (\ie in terms of
the semantics of the code).  
%Since the goal of our work is to improve the soundness of the security
%analysis approaches under study, we must consider how to most
%effectively instantiate operators from their definitions. 
We consider taking an adversarial stance to implementing security
operators, i.e., with the objective of instantiating operators to evade
detection, in order to create robust operator instantiations which are
more likely to find hidden assumptions contributing to the
sound\emph{i}ness of the analysis tools. 
Intuitively, one might consider taking
an {\em adversarial} stance to implementing security operators, in which
program mutations are introduced with the intent of evading detection.
This would result in {\em strong} operators that are more likely to
reveal unknown assumptions contributing to the sound\emph{i}ness of the
analysis tools. Given the established methodology of our empirical
analysis, we plan to leverage the opportunity to extract potential
adversarial examples of operators in a data-driven manner. The PIs have
currently obtained access to two widely-used sources of Android Malware:
the Android Malware Genome Project~\cite{zj12} (1,260 samples) and the
Android Malware Dataset~\cite{wlr+17} (24,553 samples), which will be
used to extract malware descriptions, application code, and other
metadata into the open coding web-app.  %The source code will be
%displayed in an interactive manner so taggers can navigate through the
%source files directly from the web-app. 
\end{comment}

The final output of this phase will be a taxonomy of high-level security
operator (\ie specifications) for Android static analysis tools, augmented with adversarial examples of malicious
implementations. 
%In particular, the extracted information will be organized into
%discrete documents (\eg bug reports, malicious code, \etc) so that they
%may be manually validated and analyzed.  The documents will be equally
%and randomly distributed among the taggers, ensuring that each document
%was classified by two taggers. The goal of the tagging process will be
%different for different data sources.  For the {\em top-down} and {\em
%bottom-up} data sources, taggers will be tasked with assigning a
%succinct high-level description of the tool claim or security bug (\eg
%data exported via network).  The tagging of the malicious code samples
%will occur {\em after} this initial round of coding, and participants
%will be asked to (i) identify specific snippets of malicious code, and
%(ii) decide whether these snippets serve as an implementation instance
%of an existing security operator, or represents a new operator. The
%manual tagging process will be supported by a Web application that we
%developed to classify the documents (\ie to describe the reason behind
%the bug) and to solve conflicts between the taggers that was
%successfully utilized in the PIs past work \cite{lbt+17}. Each
%participant will independently tag the documents assigned to them.
%Every time the participants tag a document, the Web application will
%display the list of tags created so far, allowing the tagger to select
%one of the already defined tags. Although, in principle, this seems to
%contradict the notion of open coding, in our proposed context, where
%the number of possible tags (\ie cause behind the bug) is extremely
%high, such a choice helps using consistent naming and does not
%introduce a substantial bias. After manually tagging all the documents,
%all the evaluators will meet to refine the identified tags by merging
%those that are similar and splitting those that are generic when
%needed.  The final output of this Task will be a taxonomy of high-level
%security operators for Android static analysis tools, where the initial
%taxonomy is augmented with adversarial examples of malicious
%implementations.

%\DENYS{We can remove this paragraph as we already talked about it} In cases for which there is no agreement between the two evaluators, the document will be automatically assigned to an additional evaluator. This process will continue until all the documents are classified by the absolute majority of the evaluators with the same tag. If there is no agreement after all evaluators tag the same document, the PIs will manually analyze these cases in order to solve the conflict and define the most appropriate tag to assign. It is important to note that the Web application will not consider documents tagged as \emph{false positive} (\eg an issue report that does not report an actual bug in a static analysis tool) in the count of the documents manually analyzed.

%In order to build a taxonomy of high-level security operator specifications, the identified tags will be clustered in cohesive groups at two different levels of abstractions, \ie categories and subcategories corresponding to the root cause and the potential tools to which they might correspond. Again, the grouping will be performed over multiple iterations, in which tags are moved across categories, and categories are merged/split.  


 %--------------Task-3----------------
\subsubsection{Assignment of Security Operators to Tools}
The result of the systematic literature review and empirical study
described above is a taxonomy of
high-level descriptions of
(i) claimed tool capabilities and
assumptions and (ii) instantiations of the programmatic patterns in adversarial examples.
Since the analyzed tools tend to extend the functionalities
of one another, there may be implicit functionalities not explicitly
mentioned in the corresponding publications or repositories.  However,
in order for security operators to be instantiated within \tool, these
explicit links need to be established, forming a hierarchy with tools at the top, operator specifications in the middle, and potential instantiations of these operators in
malicious code segments at the bottom. %forming a hierarchy consisting of (i) tools, (ii) tools' functionalities and applicable operators from
%security bugs, and (iii) potential instantiations of these operators in
%malicious code segments.
To form this hierarchy, which will be used
to instantiate the derived operator specifications, we conducted a
final round of open coding.  During this final coding round, our extracted operators
were coded by the authors.


\subsection{Mutation Scheme}
\label{sec:mutation_scheme}
%\ADWAIT{Should we rename this to Mutation Scheme? Policy sounds cool,
%but some security people may confuse it with the more specific security
%policy, which is completely unrelated. Thoughts?}

To enable the security evaluation of Android static analysis tools,
\tool must implement mutations within Android apps.  
Mutating Android apps requires instantiating
security operators derived previously, but in the context of the security tool
being evaluated.
This will be followed by injecting the mutations (\ie instantiated
operators) at one or more locations in the app's code.
The specific method for instantiating mutations and placing them within
Android apps form the mutation placement scheme. 
\begin{comment}
We will design multiple such mutation schemes, and evaluate their
effectiveness using existing  metrics used in mutation testing of
general software, while extending existing metrics or defining new
metrics specifically for use in security. 
\end{comment}
%This major thrust of developing and analyzing
%mutation schemes, will be initially investigated considering one
%category of tools (\ie data leak detection tools), and its generality
%will be explored in later tasks (\ie {\em Task 8}).

% Task: Implementing mutations
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figs/instantiation}
  \caption{{\small A security operator may be instantiated differently
  based on the security tool being evaluated. As shown here, a
  network export security operator may be instantiated to express {\sf
  (1)} the leak of private data for evaluating FlowDroid~\cite{arf+14},
  or {\sf (2)} the use of vulnerable API, for evaluating
  MalloDroid~\cite{fhm+12}.}}  
  \label{fig:instantiation}
\end{figure}

\subsubsection{Operator Instantiation}
Security operators are abstract constructs that may apply to more than
one type of security tool from the taxonomy described in
Section~\ref{sec:operators}.  Hence, we need to automatically
generate different tool-specific implementations of the same security
operator, for evaluating different tools with \tool.  For instance,
consider the operator to ``export data via a network connection'' shown
in Figure~\ref{fig:instantiation}.  For evaluating a tool that detects
private data leaks (\eg FlowDroid~\cite{arf+14}), we may need multiple
instances of this operator, \ie mutations, to express the various kinds
of private data that can be acquired from the device using Android's API
and exported via one or more APIs for creating an Internet connection.
However, for evaluating a tool that finds vulnerable SSL
connections (\eg CryptoLint~\cite{ebfk13}), we may want the mutations to
express the use of vulnerable SSL API (\ie of SSL classes that can be
overridden, such as a custom TrustManager that trusts all
certificates~\cite{badtrustmanager}).  Therefore, when instantiating
mutants from security operators, it is imperative to consider the
context of the security tool being evaluated.

The context needed for instantiating operators may be derived from the
tool's security goals.  For example, FlowDroid's security goal is to
detect data leaks, which is why the instantiation of the network export
security operator in FlowDroid's context must consider various private
data {\em sources} and public {\em sinks}. Since the security goals of
the tool will already be expressed in our taxonomy from {\em Task 1},
the task is then reduced to automatically extracting this context from
the tool's security goals. 
%We will leverage insights from our preliminary investigation for this
%purpose.  
Moreover, since tools of
the same type have common security goals, we may be able to extract the
context in common for a large set of tools belonging to the same type.
This is advantageous for two reasons: (i) \tool gets improved
coverage in terms of potential operator instantiations, since instances
generated over an entire category of tools represented by their security
goal are applied to individual security tools, and (ii) the task of
instantiating operators bears only a one-time cost when performed for
the security goal.

One of the key insights of \tool is that the
context of a security tool can be derived from its security goals, which
are often precisely specified in configuration files; \eg we used
FlowDroid's~\cite{arf+14} sources and sinks file to instantiate mutants
that acquired data from sources and exported to sinks.  
\begin{comment}
Additionally, we
explored 36 tools from the taxonomy of Android security techniques
described by Reaves et al.~\cite{rbg+16} for goal-related configuration
files. We found that out of nine categories (\ie by goal, thus excluding
the ``other'' category), research tools have been developed for six. Our
of these six categories, we confirmed that four had at least one (in
most cases more than one) tool that provided a configuration file. In
the cases where there was no configuration file, we encountered two
possibilities: (i) one could be easily developed, given the simplicity
of the tool (\eg MalloDroid~\cite{fhm+12}), or (ii) we had no
observations as the tools were not open source and the papers were
unclear about configuration. To summarize, our preliminary work
demonstrates that for most security goals surveyed by prior work, the
security context is often explicitly precisely specified in
configuration files.
\end{comment} 
\begin{comment}
As described in
Section~\ref{sec:preliminary}, our manual investigation of
FlowDroid~\cite{arf+14} used FlowDroid's configuration file (\ie,
sources and sink file), which contains private data sources (\ie data
access APIs) and all potential sinks (\eg network/storage APIs), to
create mutations in apps. A key insight here is that FlowDroid's
security goals, and the precise context (\ie in terms of mutant
instantiation), was obtained from this configuration file. In addition
to this, we also explored 36 tools from the taxonomy of Android security
techniques described by Reaves et al.~\cite{rbg+16} for goal-related
configuration files. We found that out of 9 categories (\ie by goal,
thus excluding the ``other'' category), research tools have been
developed for 6. Our of these 6 categories, we confirmed that 4 had at
least one (in most cases more than one) tool that provided a
configuration file. In the cases where there was no configuration file,
we encountered two possibilities: {\sf (1)} one could be easily
developed, given the small number of code artifacts (\eg
MalloDroid~\cite{fhm+12}), and {\sf (2)} we had no observations as the
tools were not open source and the papers were unclear about
configuration. To summarize, our preliminary work demonstrates that for
most security goals surveyed by prior work, the security context is
often explicitly specified in terms of configuration files.
\end{comment}
\begin{comment}
We performed a manual investigation of
FlowDroid~\cite{arf+14}, during which we instantiated the security
operator that exports data to the network. 
The key observation during our
analysis was that FlowDroid uses a configuration file that has a list of
private data sources (\ie data access APIs) and all potential sinks
(\eg network/storage APIs), which is claimed as comprehensive in the
documentation. This configuration file thus represents the security
goals, and hence the context, of FlowDroid. As a result, in our
preliminary investigation, we could easily use this file of sources and
sinks to instantiate the ``export data via the network'' security
operator. \TODO{Further, we studied the rough taxonomy of security tools
developed by Reaves et al.~\cite{stardroid}, and confirmed that at least
\xy security tools that detect information leaks have security goals
that can be expressed with the configuration file containing sources and
sinks.} \TODO{Finally, we also investigated other types of tools (\eg
SSL API verification tools), and discovered that there are already
existing configuration files that may represent the security goals, or
that the configuration files can be created using text analytics with
manual supervision.}


Security tools that check for
vulnerabilities or malware are often configurable (\ie instead of having
hard-coded checks), and the configuration files may offer a precise
representation of their security goals. We will investigate the use of
configuration files for instantiating mutations from security operators.
For each broad category of tools derived from our taxonomy (\eg data
leak detection tools), we will generate a single, comprehensive,
configuration file by combining the configurations of tools from that
category. We will record the feasibility of doing so, and where
required, will apply text analytics (as in our prior work
\cite{Linares-Vasquez:ICPC:2014,Cortes-Coy2014,Vendome:ICSE17,Le:ICPC15:2})
on tool documentation in addition to manual effort. We will then develop
methods to transform each security operator that applies to the tool
category into executable mutant instances using this configuration file
with the app mutation techniques from our prior work ~\cite{lbt+17}. For
instance, the mutant instances for FlowDroid shown in
Figure~\ref{fig:instantiation} may be derived by applying the sources
and sinks in the configuration file to ``data'' and ``network
connection'' fields of the security operator specification respectively.
As described previously, that generated category-specific configuration
file may be more comprehensive than individual tool configurations, and
cost less effort to create and maintain.
%The generated category-specific configuration file may be more
%expressive than individual tool configurations, and hence will expand
%the coverage of our instantiation, while reducing the cost to a one-time
%effort.  
Finally, we will increase the expressiveness of \tool by
augmenting this context-specific corpus of instantiations with
adversarial instantiations created at the end of {\em Task 2}.
\end{comment}
% Operators can be abstract; \eg export private data to the network,
% export private data via bluetooth
% Need to implement specific mutants. How?
% Insight: Tools provide policy files that are precise representations of their security goals.
% Proposed work: Not much remains really. Need to think more on this.

% Based on the security Goals. Therefore, the context is in the security
% goals, often represented by config files. Since the security goals are
% similar for an entire group of tools, we may be able to use a broad
% collection of config files on every tool of that type, allowing broad
% coverage with a one-time optimum effort.

% Task: Placing mutations
\subsubsection{Mutant Placement}
The placement of mutation instances in the target Android app is
an important task that directly affects the expressiveness and
effectiveness of the mutation scheme. Naive placements (\eg in the first
block of the app's code)) are generally discouraged, as they are
always detected, and hardly test the effectiveness of the tool being
evaluated~\cite{DaranT96,Andrews:ICSE05,AndrewsBLN06,Just:FSE14}; While
previous mutation tools typically injects mutations into all potential program insertion
points \cite{Ma:2005,Jester,Just:ISSTA14,Jumble,PIT,Schuler:FSE09}, 
{\em this proposal is first to
consider the challenges of seeding
mutants for effectively evaluating security tools}. 

% Explain this better:
% Security must go beyond functionality: \ie functionality testing
% detects change in desired functionality. Security testing detects
% functionality that is identical to the desired functionality, but
% which may still violate some security goals.
% The security tool lacks the ``observation'' of missing functionality
% (\ie a functionality testing tool observes a difference in the
% desired functionality).
One important challenge (and distinction) is the need to assume an
adversarial setting when evaluating security tools. Consider this
argument from Section~\ref{sec:background}. When using mutation testing
for software testing, a software test suite is scored based on how many
mutants it detects. However, during security-oriented mutation testing,
the number of mutants caught by the security tool are immaterial;
instead, the mutants that are not detected matter, and must be resolved
to design/implementation flaws. Given many such semantic
differences (see Section~\ref{sec:background}), existing mutation
placement techniques for functional mutation analysi may not be applicable for
security.  Instead, mutation placement strategies for security must also
consider the adversarial nature of the problem space (\ie adversary
models) while seeding mutants.

\begin{comment}
For example, a functionality testing tool is deemed effective if it
exercises the mutated code, thereby leading to a difference in the
output of the mutant and the original program.  However, a security tool
must not only reach the mutated portion(s) of the program, but also
detect the mutation (\eg MalloDroid~\cite{fhm+12} must detect vulnerable
SSL API). As a result, the security tool must detect functionality that
is identical to the desired app functionality, but which may be
suspicious in certain contexts, dependent on the tool's security goals;
e.g, exporting data is perfectly legitimate functionality, but a
security tool must differentiate between exports of confidential and
non-confidential data.  As a result, the existing mutation placement
techniques for functionality may not be applicable for security.
Instead, mutation placement strategies for functionality must also
consider the adversarial nature of the problem space (\ie must consider
adversary models while seeding mutants).



In our preliminary investigation in Section~\ref{sec:preliminary}, we
manually placed mutations at random locations in an open source Android
app. While this random strategy does not consider an adversarial
scenario, it was more effective than a trivial placement of mutants,
\ie  a trivial approach may have never placed the mutation in the code
of an Android fragment.  Further, Android's application model and other abstractions
must also be considered for effective mutant placement in Android apps. 
% Can elaborate on Android's peculiarities if needed
Our strong preliminary work on seeding mutants in
\mplus~\cite{lbt+17} lays the groundwork for further exploration.
\end{comment}

%\DENYS{We talk about machine learning at the beginning of 4.1 for task
%5 ("For this task, we will use machine learning to extract patterns of
%the desired mutation(s) from a diverse array of real trusted
%applications (\ie to devise the mutation schema for accidental
%disclosure), and separately from malware samples that leak information
%(\ie to devise the mutation schema for malicious disclosure).") but I
%do not think we have any details or mentions here:}
% What?
As a first step towards this adversarial mutant injection we automate random mutation placement for Android
apps within \tool. \KEVIN{We need some more information here.}

\begin{comment}
Following this, we will develop more nuanced mutant
seeding strategies considering two specific adversaries based on their
motivations: (i) curious/benign apps, and (ii)
malicious apps.
That is, when evaluating a security tool, we want to examine if the tool
can detect mutations {\em as they occur (\ie as per their locations)} in
benign apps, as well as those in malicious apps.  
% Why?
Importantly, each strategy also serves to facilitate a specific use case
that motivates \tool~(Section~\ref{sec:impacts}).  
% Why?
First, we will to improve the guarantees developers get when they
evaluate their own apps for accidental vulnerabilities using
existing tools, by designing a mutation placement strategy that accounts
for mutation locations in existing benign apps. Our prior work
(Aquifer~\cite{ne13}) motivates this strategy, by highlighting the
importance of addressing accidental data leaks (and other
vulnerabilities by extension) in Android apps.  Second, we will
improve the guarantees obtained by security researchers when they test
apps for malicious behavior using existing tools, by similarly
designing a mutation strategy that accounts for mutation locations in
known malware.  
% How?
To model our strategies after the locations of security operators in
malicious or benign apps, we will identify the locations of code clones
of the operator instances defined in \textit{Task 4} in a  diverse set
of real apps.  As the operator instances defined in \textit{Task 4} may
not be syntactically equivalent to similar functionality found in
apps/malware, we will leverage our prior work on detecting functionally
equivalent code clones that are syntactically dissimilar~\cite{wtvp16}.
Once these \textit{general} benign and adversarial mutant location
patterns have been identified, \tool will utilize Abstract Syntax Tree
(AST), and textual analysis to seed mutations into similar locations in
target apps (See Sec 4.4).  To support this methodology, we have
acquired access to a dataset of more than {\em 4 million}
apps~\cite{abkl16} and {\em 24,556} malware samples~\cite{wlr+17}. We
will augment \tool with additional malicious and benign app samples as
they become available.   Developing mutation placement strategies based
on our observations in different adversaries will allow \tool to perform
a robust analysis that supports a diverse set of adversarial use cases.
\end{comment}

% Placing mutants correctly is important. We want to maximise effectiveness.
% For \tool, effectiveness means being able to find as many bugs in the security tool being evaluated as possible, \ie maximum coverage.
% This is challenging: different from the general definition in the context of software mutation testing, where we want to find bugs in the software being mutated itself.
% Our intuition, use security goals to motivate strategies for location placement
% 1. Can \tool find leaks in benign apps? Dev wants to test own app for accidental disclosure. Proposed work: Test with a diverse corpus of real applications. Use sources/sinks, \ie place sinks after existing sources, at different intervals, based on static analysis, to simulate real leaks.
% 2. Can \tool find leaks in malicious apps? Proposed work: (a) Random placement for brute force coverage (\ie place source-sink pairs randomly everywhere), (b) mimic malware, \ie study where leaks occur in malware.

% Task: Placing mutations
\begin{comment}
\task{Scheme Metrics}
% Task: Evaluating mutation implementation and placement: 
% Which is more effective? How to measure effectiveness? Use existing
% metrics in mutation testing, and develop new ones specific to
% security. Redefine existing metrics (stillborn, trivial) in the
% security context, or create new ones if required.

Placing mutation operators

Implement mutation operators: sources and sink files, make abstract
operators (export data) real (get source, export sink).
Evaluate random placement
Design Type-specific Strategies for placing operators: Insight: We may
be able to automatically get some sense of how to implement the
operator, and where, based on the policy files often accompanying those
tools. E.g., FlowDroid Sources and sinks: Mutant is getSource,
exportSink combo.
Can it detect Accidental/benign/curious app: Can start looking wherever
getSource occurs in an existing real applications, and place exportSink
at multiple points in code after. Large corpus of diverse apps.
Malicious app: Can use source/sink combos at different locations, or
random locations not explored by ordinary apps, or where they ordinarily
don't exist in benign apps.
\end{comment}

\begin{comment}
\subsection{Core Expansion}

\subsubsection{Data Privacy} 
The security goal of preserving user data privacy has been one of the
most prominent subjects in smartphone security with a large number of tools for Android app
analysis~\cite{arf+14,gcec12,akg+15,ralb14,lbb+15,old+15,kfb+14,gkp+15,gzjs12,svt+14,llw+12,lkm+13,xtf+15,eyr12,fada14}.
Thus, this category of tools forms the first subject of our analysis.
\end{comment}
%Thus, we focus on this category of tools first.
\begin{comment}
Our preliminary work initiated a manual investigation of
FlowDroid~\cite{arf+14}, and detected a vulnerability, which was not
described in the paper. We plan to continue using \tool in this
direction.
\end{comment}

\begin{comment}
We will evaluate the soundness of publicly available data leak detection
tools that use static analysis for modeling or tracking information
flows in Android
apps~\cite{arf+14,gcec12,akg+15,ralb14,lbb+15,old+15,kfb+14,gkp+15,gzjs12,svt+14,llw+12,lkm+13,xtf+15,eyr12,fada14}
using \tool, starting with FlowDroid~\cite{arf+14}. Upon finding a
vulnerability, we will expand our investigation to other security tools
that extend the tool in question, \ie we will use the information
obtained from our systematically derived tool taxonomy in the literature
review in \textit{Task 1}, and recursively initiate an investigation of
any other tool that inherits or extends the current tool in question.
This is important, as research tools may extend the functionality of or
inherit other publicly available tools, in turn also inheriting their
vulnerabilities. For instance, none of the 13 tools that extend
FlowDroid discuss the fragment bug discovered in our preliminary work,
which demonstrates a large likelihood of vulnerability propagation.
However, instead of solely relying on the documentation, we will
evaluate the derivative tools with \tool, to help confirm the
vulnerability propagation.


% 8 research tools, evaluate them
% see what all tools are affected
\subsubsection{Vulnerability Resolution}
\tool will assist developers and security researchers alike in
finding flaws (\ie uncaught mutants) in
security tools. However, it is important to resolve the flaw to
a design choice, implementation decision or assumption in the tool, in order
to systematically address all root causes of the flaw. Finding the root causes and assumptions behind flaws
will eventually allow us to assist developers in fixing the
flaws, and expanding the sound core of their tools, as shown in Fig.~\ref{fig:expanding_core}. The quantity of fixed
(unique) flaws will be one success metric for \tool.
% bug reports
% help them track the source of the bug
% --> developing a patch is a course project in mobile application security
% --> even develop patches in some cases where we might be familiar.
% formally track the response
% success metric

As described in our preliminary investigation in
Section~\ref{sec:preliminary}, we observed that the FlowDroid did not
detect a particular mutation. While the mutation itself did not
provide any information on the actual cause behind the flaw, we
performed additional analysis and {\em resolved the cause behind this
flaw} to FlowDroid's incorrect modeling of Android's fragments.
We have informed the authors of this flaw, and are currently
assisting them to diagnose and fix it.

%As described in our preliminary investigation in
%Section~\ref{sec:preliminary}, we observed that the FlowDroid did not
%detect one particular mutation. The mutation itself did not provide any
%information on the actual cause behind the flaw. On further
%manual analysis, we {\em resolved the cause behind this flaw}
%and discovered that FlowDroid did not account for Android's fragments.
%We have informed the authors of this flaw, and are working with
%them to diagnose and fix it.

We will report the flaws we find
to the respective tool developers. The flaw report will contain
information on the specific mutants that the tool failed to detect, and
its properties (\eg location within the target application, the
security operator, the actual code). Using this information, we will
assist developers in resolving the flaws to assumptions or
decisions in the tool's design or implementation, and contribute patches
wherever possible. Further, the resolution of flaws and
development of patches may also serve as educational activities in the
relevant classes taught by the PIs. For instance, PI Nadkarni teaches an
undergraduate class on ``Mobile Application Security'', and the task of
developing patches for known flaws in publicly available
Android security tools may be assigned as a course project. After
disclosing the flaws to the concerned developers, we will
formally track flaws and responses (\eg by submitting bug
reports) and make our data available for the research community and end
users as a whole. This open catalog of unsound assumptions in existing
tools will allow end-users to form realistic expectations about the
security of the analysis performed using these tools.

\subsubsection{Security Goals and Refinement} 
Our initial investigation will target tools that detect private data
leaks, primarily due to the large number of available tools and significant impact of such tools. However, we
envision that the comprehensive tool taxonomy and security operators
developed as a part of the first phase of this proposal will provide an
opportunity to explore our methodology in the context of other types of
tools, which satisfy other important security goals.  There are a few
other pressing security concerns that may form excellent candidates for
an evaluation with \tool; for instance, tools that detect SSL
vulnerabilities(\eg MalloDroid~\cite{fhm+12} and
CryptoLint~\cite{ebfk13}).  Using \tool with a different category of
security tools will serve as a stress test for \tool, and as a way to
gauge the limits of mutation testing in security evaluations. 

We will evaluate other types of security
tools, such as SSL vulnerability detectors, using \tool. For this, we
will replicate our methodology for instantiating operators in the
context of the specific tool or tool category ({\em Task 4}), and
determining mutation placement ({\em Task 5}) for the security goal of
the tool.  Further, to prioritize our efforts, we plan to organize
surveys among researchers in the security community to determine what
category of tools deserve most or immediate attention. We will
collaborate with experts and/or developers of specific security tools as
well as our industrial partners (see support letters) to develop better
security operators and mutation policy.  In this regard, we have already
received an intent to collaborate from Dr. Bradley Reaves, a security
expert in the area of SSL verification tools, and a developer of a tool
for analyzing SSL use in mobile money applications~\cite{rsb+15}.
Finally, we will engage the security and SE communities to improve \tool
(\eg by allowing developers to add new security operators absent in
\tool), and to explore future directions in the use of mutation testing
for evaluating security tools (\eg by organizing
briefings/tutorials/working sessions co-located with conferences).
Sharing the valuable insights acquired from evaluating entire categories
of security tools with the security and SE research
communities, and engaging them in improving \tool, is one of
the high-level objectives of this proposal.

%Finally, evaluating security tools with \tool will help us acquire
%valuable insights into the use of mutation testing for security. Sharing
%these insights with the security and software engineering
%research communities, and engaging them in improving \tool, is one of
%the high-level objectives of this proposal.

% SSL Vulns, other tools
% Refinement of the tool, identify limitations in terms of generality
% Improve operators, instantiations
% Organize a workshop; Technical briefing, working session, at ASPLOS
% Survey in the security community --> where to prioritize?
% Engage the community (\eg allow people to submit operators that we
% have missed

%\task{Refinement}
% Organize a workshop; Technical briefing, working session, at ASPLOS
% Survey in the security community --> where to prioritize?
% Engage the community (\eg allow people to submit operators that we
% have missed
\end{comment}



==> background.tex <==
\section{Background on Mutation Analysis}
\label{sec:background}

Formal verification of soundness guarantees in software, while an ideal
approach, is one of the most difficult problems in computer security. For
instance, prior work on formally verifying apps or systems often
requires the monitor to be rewritten in a new programming language or
uses verification-specific programming constructs (\eg verifying
reference monitors~\cite{fcds10,vcj+13}, information flows in
apps~\cite{mye99,ml00,yys12}), which poses practical concerns for tools
based on numerous legacy codebases (\eg FlowDroid~\cite{arf+14},
CHEX~\cite{llw+12}). Further, formal verification techniques generally
require correctness to be specified, \ie the policies or invariants
that the program is checked against. Concretely defining what is
``correct'' is hard even for high-level program behavior (\eg making a
``correct'' SSL connection), and may be infeasible for complex static
analysis tools that analyze apps (\eg detecting ``all
incorrect SSL connections'').  To the best of our
knowledge, there has been no prior attempt at formally verifying the
soundness of security-focused Android static analysis tools. Hence, this
paper investigates a more practical (and feasible) approach of systematically
evaluating security tools using mutation testing, which gradually
improves security tools and brings them closer to performing a fully-fledged sound
analysis.

\begin{comment}
In this section we outline background concepts and related work from three different areas; (i) mutation analysis from the perspective of software testing, (ii) verification of security-focused program analysis tools, and (iii) static analysis tools for Android.  For each area we discuss the relevance of concepts and distill the novelty of our proposed research. %We do not discuss literature related to the functional testing of Android apps \cite{Amalfitano:ASE12,Hao:MobiSys14,Mahmood:FSE14,Machiry:FSE13,Shauvik:2015,Linares:MSR15,Moran:ICST16,Mao:ISSTA16,Linares-Vasquez:ICSME17}, as this is not the direct goal of the work set forth in this proposal.
For further details about the concepts, recent research, and future work in the field of mutation testing, one can refer to the survey by Jia and Harman~\cite{Jia:TSE}.
\end{comment}

Mutation analysis or testing has a strong foundation in the field of Software Engineering.  The process of mutation analysis is succinctly
defined by Offutt and Untch, \textit{``[Mutation analysis
proceeds by inducing] faults into software by creating many versions of
the software, each containing one fault. Test cases are used to execute
these faulty programs with the goal of distinguishing the faulty program
from the original program"} \cite{Offutt2001}.  Mutation analysis is
typically utilized as a test adequacy criterion, measuring the
effectiveness of a set of test cases.  A larger number of faulty
programs or \textit{mutants} detected by a test suite, indicates a
higher effectiveness for that particular test suite.  Faulty programs
are created by applying transformation rules, called \textit{mutation
operators} to a correct program.  Since the introduction of mutation
testing in the 70s~\cite{Hamlet:TSE,DeMillo:Computer}, researchers have
tried not only to define new mutation operators for different
programming languages and paradigms (Java \cite{Ma:ISSRE03} and Python \cite{Derezinska2014}), but
also for specific types of software like Web applications
\cite{Praphamontripong:Mutation15} and data-intensive applications
\cite{Appelt:ISSTA14,ZhouF09} to exercise their GUIs
\cite{Oliveira:ICSTW15} or to alter model-based input data
\cite{Nardo:ICST15}.  Recently, mutation analysis has been applied to
measure the effectiveness of test suites for both functional and
non-functional requirements of Android apps, including preliminary work
on a tool called \mplus \cite{Deng:ICSTW15,Jabbarvand:FSE17,lbt+17}.


The research outlined in this paper builds upon the theoretical
underpinnings of mutation analysis from the SE community
and instantiates them in a security-focused context. Our methodology does not
simply use the traditional mutation analysis process, but rather {\em
redefines} this methodology to effectively improve the soundness of
security-focused static analysis tools. For instance, in the context of
software testing, a test suite is considered to be effective based on the
number of mutants it detects. However, in our context of
evaluating security-related soundness, mutants represent behaviors that \textit{should} be detected. Thus rather than focusing on a mutation score, our analysis is concerned with mutants that are
not detected, so that they may be linked them back to unsound design or implementation
choices, in order to then fix the security tool. 

Further, we design and
instantiate {\em security operators}, which at an abstract level are
similar to mutation operators (\ie they are transformations applied to
end-user apps, resulting in mutants). However, their derivation
and instantiation both significantly differ from traditional mutation
operators. That is, deriving the specifications for a rich set of
security operators requires understanding of the security goals and
claims of a diverse body of static analysis security techniques, which is not a
traditional requirement in mutation testing. Further, the instantiation
of security operators must often be in the context of the security
technique being evaluated.  Similarly, while
functional metrics are considered when seeding mutants in software
testing, our research considers seeding strategies based on different
adversarial models. In summary, while we transform the traditional process of
mutation analysis for our research goals, we retain its key benefit of
illustrating the limitations in the artifact it is used to evaluate,
which in our context are security-focused Android static analysis tools,
rather than test suites. %Therefore, our work can take advantage
%of the engineering infrastructure generated by prior work in
%mutation testing of Android apps by the co-PI~\cite{lbt+17}.

%\ADWAIT{Do we even need a static analysis section? We have already
%described the soundiness argument in the intro, and given numerous
%examples of Android tools:
%Mathis \etal recently introduced an approach that relies on mutating
%input data, and detecting the mutated data in identified sensitive sinks
%in Android apps. This approach was able to 75 information flow paths
%that {\sc \small FlowDroid} missed.  
%}
%\DENYS{I think this section is good, we do not need to talk about static analysis tools here}


\begin{comment}
In the context of this proposal, security operators are code
transformations applied to end-user Android apps resulting in mutants.
Static analysis approaches for detecting security vulnerabilities are
then run on the resulting mutants, rather then the mutants being run
against a functional test suite.  Our intuition is that by designing
security operators that apply transformations intended to evade
detection by static analysis tools, undiscovered limitations and
assumptions in these tools can be detected and documented.  Thus,
whereas in traditional mutation analysis undetected mutants signal
limitations of a test suite, undetected mutants born of security
operators indicate potential important assumptions impacting the
soundness of security-focused static analysis approaches. In summary,
while we modify the traditional process of mutation analysis for our
research goals, we retain its key benefit of illustrating limitations in
the construct it is applied to evaluate, which in our context are static
analysis tools rather than test suites.
\end{comment}
\begin{comment}
Changes induced by mutation operators are typically relatively simple,
due to a concept called the \textit{coupling effect} that states that
\textit{"complex faults are coupled to simple faults in such a way that
a test data set that detects all simple faults in a program will detect
most complex faults."}  The extent to which this coupling effect applies
to real world software is a subject of active study, particularly from
the point of view of whether mutants are \textit{representative} of
naturally occurring real faults
\cite{DaranT96,Andrews:ICSE05,AndrewsBLN06,Just:FSE14}.  
\end{comment}

	%In addition to functional mutation tools such as
	%$\mu$Java~\cite{Ma:2005}, Jester~\cite{Jester},
	%Major~\cite{Just:ISSTA14}, Jumble~\cite{Jumble}, PIT~\cite{PIT}
	%and javaLanche~\cite{Schuler:FSE09}, there has been recent work
	%related to deriving functional and non-functional mutation
	%operators and operationalizing mutation analysis for the
	%Android platform. Deng \etal, \cite{Deng:ICSTW15}, defined
	%eight mutation operators aimed at introducing faults in the
	%essential programming elements of Android apps, \ie intents,
	%event handlers, activity lifecycle, and XML files (\eg GUI or
	%permission files). Recent work by the PI on \mplus builds upon
	%Deng \etal's work by empirically deriving a total of 36 novel
	%mutation operators tailored for the Android platform derived by
	%semi-automatically analyzing information gleaned via mining
	%software repositories and user reviews. Jabbarvand and Malek
	%introduced $\mu$Droid \cite{Jabbarvand:FSE17}, a mutation
	%testing framework for the non-functional software quality
	%attribute of energy usage.  %Their framework utilizes a novel
	%energy estimation oracle and several empirically derived
	%energy-focused operators.  This recent work related to Android
	%illustrates that effectiveness that mutation testing can
	%achieve for non-functional software requirements, and serves as
	%a point of inspiration for the proposed work. 

%Daran and Th\'evenod-Fosse \cite{DaranT96} were the first to
%empirically compare mutants and real faults, finding that the set of
%errors and failures they produced with a given test suite were similar.
%Andrews \etal \cite{Andrews:ICSE05,AndrewsBLN06} studied whether
%mutant-generated faults and faults seeded by humans can be
%representative of real faults. The study showed that carefully-selected
%mutants are not easier to detect than real faults, and can provide a
%good indication of test suite adequacy, whereas human-seeded faults can
%likely produce underestimates. Just \etal \cite{Just:FSE14} correlated
%mutant detection and real fault detection using automatically and
%manually generated test suites. They found that these two variables
%exhibit a statistically significant correlation. At the same time,
%their study pointed out that traditional Java mutants need to be
%complemented by further operators, as they found that around 17\% of
%faults were not related to mutants (i.e., due to algorithmic changes
%and code deletion). 

	
%Most of the available mutation testing tools are in the form of
%research prototypes. Concerning Java, representative tools are
%$\mu$Java~\cite{Ma:2005}, Jester~\cite{Jester},
%Major~\cite{Just:ISSTA14}, Jumble~\cite{Jumble}, PIT~\cite{PIT}, and
%javaLanche~\cite{Schuler:FSE09}. Some of these tools operate on the
%Java source code, while others inject mutants in the bytecode. For
%instance, $\mu$Java,  Jester, and Major generate the mutants by
%modifying the source code, while Jumble, PIT, and javaLanche perform
%the mutations in the bytecode. Tools for mutation testing can be also
%categorized according to the tool's capabilities (\eg the availability
%of automatic tests selection). A thorough comparison of these tools is
%out of the scope of this paper. The interested reader can find more
%details on PIT's website \cite{MutationTools} and in the paper by
%Madeysky and Radyk~\cite{Madeyski:IET10}. Several researchers have
%proposed approaches  to measure the effectiveness and efficiency of
%mutation
%testing~\cite{Offutt:1991,Andrews:ICSE05,Gopinath:ICSTW16,Just:ICST12}
%to devise strategies for reducing the effort required to generate
%effective mutant
%sets~\cite{Adamopoulos:2004,Just:ISSTA14-2,Gopinath:ICSE16}, and to
%define theoretical frameworks~\cite{Jia:TSE,Shin:ICST16}. Such
%strategies can complement our work, since in this paper we aim at
%defining new mutant operators for Android, on which
%effectiveness/efficiency measures or minimization strategies can be
%applied.

\begin{comment}
%\KEVIN{@Adwait, I realized that in both our security-focused static
analysis approach and in traditional mutation testing, undetected
mutants signal problems}%Furthermore, we assert that specifications for
mutation operators can and should be empirically derived from documented
functional claims of security-focused static analysis tools and security
bugs in open source apps. More specifically, by applying security
focused mutation operators to Android apps that are analyzed by static
analysis tools, it should be feasible to uncover deficiencies in these
tools.  While mutation testing frameworks for Android apps related to
both functional and non-functional goals have been proposed, none of
these approaches are security focused.  Our proposed work has the
potential to improve both the soundness of security-focused static
analysis tools and end-user apps, ushering in a new direction of cross
cutting research in both SE and computer security that utilizes mutation
analysis to vet security-focused program anValysis tools and various security-related requirements of software.
\end{comment}

